Universality for the directed configuration model: metric space convergence of the strongly connected components at criticality

We consider the strongly connected components (SCCs) of a uniform directed graph on $n$ vertices with i.i.d. in- and out-degree pairs distributed as $(D^-,D^+)$, with $\mathbb E[D^+]=\mathbb E[D^-]=\mu$. We condition on equal total in- and out-degree. A phase transition for the emergence of a giant SCC is known to occur at the critical value $\mathbb E[D^-D^+] = \mu$. We study the model at this critical value and, additionally, require that $\mathbb E[(D^-)^i(D^+)^j]<\infty$ for all $i+j\leq 3$, and for $(i,j)=(1,3)$ and $(i,j)=(3,1)$. We show that, under these conditions, the SCCs ranked by decreasing number of edges with distances rescaled by $n^{-1/3}$ converge in distribution to a sequence of finite strongly connected directed multigraphs with edge lengths, and that these are either $3$-regular or loops. The limit objects lie in a $3$-parameter family, which contains the scaling limit of the SCCs in the directed Erd\H{o}s-R\'enyi model at criticality as found by Goldschmidt and Stephenson (2019). This is the first universality result for the scaling limit of a critical directed graph model and the first quantitative result on the directed configuration model at criticality. As a trivial consequence, the largest SCCs at criticality contain $\Theta(n^{1/3})$ vertices and edges in probability, and the diameter of the directed graph at criticality is $\Omega(n^{1/3})$ in probability. We use a metric on the space of weighted multigraphs in which two multigraphs are close if there are compatible isomorphisms between their vertex and edge sets which roughly preserve the edge lengths. We use the product topology on the sequence of multigraphs. Our method of proof involves a depth-first exploration of the directed graph, resulting in a spanning forest with additional identifications, of which we study the limit under rescaling.

==> Content/Sections/Sampling+algorithm.tex <==
\begin{algorithm}[htbp]
    \SetAlgoLined
    \KwData{A set of vertices $\{v_1,\dots, v_n\}$ with degree pairs $(d^-(v_1),d^+(v_1)),\dots, (d^-(v_n),d^+(v_n))$ satisfying $\sum d^-(v_i)=\sum d^+(v_i)$}
    $\exploredvertices \leftarrow$ an empty ordered list of vertices \tcp*[f]{the list of discovered vertices}\;
    $\edgestack \leftarrow$ an empty ordered list of vertices \tcp*[f]{the queue}\;
    $(d^-_{\mathrm{unpaired}}(v_1),\dots,d^-_{\mathrm{unpaired}}(v_n))\leftarrow (d^-(v_1),\dots,d^-(v_n))$  \tcp*[f]{the number of unpaired in-edges per vertex}\;
    $k \leftarrow 0$ \tcp*[f]{the index of the current step} \;
    $\hat{s}^- \leftarrow 0$ \tcp*[f]{the number of seen but unpaired in-edges}\;
    $\hat{s}^+ \leftarrow 0$ \tcp*[f]{the total stack size minus the number of explored out-components} \;
    $\forest \leftarrow$ a directed forest containing vertices $v_1,\dots v_n$ and no edges
    \tcp*[f]{the current out-forest}\;
     $M \leftarrow$ a directed multigraph containing vertices $v_1,\dots v_n$ and no edges
    \tcp*[f]{the current directed multigraph}\;
    \While(){there exist undiscovered vertices with positive in-degree OR $\exploredvertices$ is non-empty}{
        \eIf(){$\edgestack$ is non-empty}{
            $v \leftarrow$ last entry in $\edgestack$ \;
            remove last entry from $\edgestack$ \;
            $\hat{s}^+\leftarrow \hat{s}^+-1$\;
            $w \leftarrow$ a random vertex chosen with prob.\ proportional to $d^-_{\mathrm{unused}}(w)$\;
            add the edge $(v,w)$ to $M$\;
            $d^-_{\mathrm{unused}}(w)\leftarrow d^-_{\mathrm{unused}}(w)-1$\;
            $\hat{s}^-\leftarrow \hat{s}^--1$\;
            \eIf(\tcp*[f]{we sampled a surplus edge}){$w\in \exploredvertices$}{
            add a dummy leaf to $F$ and an edge from $v$ to the leaf\;}{
            add the edge $(v,w)$ to $F$\;
            }
        }{
        $w\leftarrow$ a random vertex not in $\exploredvertices$ chosen with prob.\ proportional to $d^-(w)$ \tcp*[f]{we start a new out-component}\;
        $\hat{s}^+\leftarrow \hat{s}^+-1$\;}
        \If(){$w\not\in \exploredvertices$}{
        append $w$ to $\exploredvertices$\;
        append $d^+(w)$ repeats of $w$ to $\edgestack$\;
        $\hat{s}^+\leftarrow \hat{s}^++d^+(w)$
        $\hat{s}^-\leftarrow \hat{s}^-+d^-(w)$
        }
        $k\leftarrow k+1$\;
        $\hat{s}^+_k\to \hat{s}^+$\;
        $\hat{s}^-_k\to \hat{s}^-$\;
        }
        
    \While(){there exist undiscovered vertices OR $\exploredvertices$ is non-empty}{
        \eIf(){$\edgestack$ is non-empty}{
            $v \leftarrow$ last entry in $\edgestack$ \;
            remove last entry from $\edgestack$ \;
            $w \leftarrow$ a random vertex chosen with prob.\ proportional to $d^-_{\mathrm{unused}}(w)$\;
            add the edge $(v,w)$ to $M$\;
            $d^-_{\mathrm{unused}}(w)\leftarrow d^-_{\mathrm{unused}}(w)-1$\;
            }{
            $w\leftarrow$ a random vertex not in $\exploredvertices$\;
            append $w$ to $\exploredvertices$\;
            append $d^+(w)$ repeats of $w$ to $\edgestack$\;
        }
        }
    
    \caption{The eDFS procedure \label{alg:edfs}}
\end{algorithm}



\begin{algorithm}[htbp]
    \SetAlgoLined
    \KwData{A set of vertices with degree pairs $(d^-(v_1),d^+(v_1)),\dots, (d^-(v_n),d^+(v_n))$ satisfying $\sum d^-(v_i)=\sum d^+(v_i)$}
    $\exploredvertices \leftarrow$ an empty ordered list of vertices \tcp*[f]{the list of discovered vertices}\;
    $\edgestack \leftarrow$ an empty ordered list of vertices \tcp*[f]{the queue}\;
    $(d^-_{\mathrm{unpaired}}(v_1),\dots,d^-_{\mathrm{unpaired}}(v_n))\leftarrow (d^-(v_1),\dots,d^-(v_n))$  \tcp*[f]{the number of unpaired in-edges per vertex}\;
    $k \leftarrow 0$ \tcp*[f]{the index of the current step} \;
    $\hat{s}^- \leftarrow 0$ \tcp*[f]{the number of seen but unpaired in-edges}\;
    $\hat{s}^+ \leftarrow 0$ \tcp*[f]{the total stack size minus the number of explored out-components} \;
    $\forest \leftarrow$ an empty directed graph
    \tcp*[f]{the current out-forest}\;
     $G \leftarrow$ an empty directed graph
    \tcp*[f]{the current directed-graph}\;
    \While(){there exist unpaired out-half-edges of vertices with positive in-degree}{
        \eIf(\tcp*[f]{we are starting a new out-component}){$\edgestack$ is empty}{
            $w \leftarrow$ a random vertex not in $\exploredvertices$ chosen with prob.\ proportional to $d^-(w)$ \;
            $\hat{s}^+ \leftarrow \hat{s}^+ - 1$ \tcp*[f]{we have finished exploring another out-component} \;
        }(){
            $v \leftarrow$ last entry in $\edgestack$ \;
            remove last entry from $\edgestack$ \;
            $w \leftarrow$ a random vertex chosen with prob.\ proportional to $d^-_{\mathrm{unused}}(w)$\;
            $d^-_{\mathrm{unused}}(w)\leftarrow d^-_{\mathrm{unused}}(w)-1$ \tcp*[f]{we have paired an in-edge of $w$}\;
            $\hat{s}^- \leftarrow \hat{s}^- - 1$ \tcp*[f]{we have paired an in-edge} \;
            $\hat{s}^+ \leftarrow \hat{s}^+ - 1$ \tcp*[f]{we have removed and edge from the stack} \;
        }
        \eIf(){$w \not \in \exploredvertices$}{
            append $w$ to $\exploredvertices$ \; 
            add the vertex $w$ to $\forest$ \;
            add the vertex $w$ to $M$ \;
            \If(){$\edgestack$ is non-empty}{
                add the edge $(v, w)$ to $\forest$\;
                add the edge $(v, w)$ to $M$\;
            }
            append $d^+(w)$ repeats of $w$ to the end of $\edgestack$ \;
            $\hat{s}^- \leftarrow \hat{s}^- + d^-(w)$ \tcp*[f]{we have discovered $d^-(w)$ new unpaired in-edges} \;
            $\hat{s}^+ \leftarrow \hat{s}^+ + d^+(w)$ \tcp*[f]{we have added $d^+(w)$ new entries to the stack}\;
        }{
            add a dummy leaf to $\forest$ and and edge from $v$ to the leaf \tcp*[f]{we have discovered a surplus edge and add a dummy leaf to the forest} \;
            add the edge $(v, w)$ to $M$\;
        }
        $k \leftarrow k + 1$ \;
        $\hat{s}^-_k \leftarrow \hat{s}^-$ \;
        $\hat{s}^+_k \leftarrow \hat{s}^+$ \;
    }
    \While(){there exist unpaired out-half-edges}{
    \eIf(){$\cQ$ is empty}
    {$w\leftarrow$ a uniformly random vertex not in $\cV$\;
    append $w$ to $\cV$\;
    add $w$ to $M$\;}
    {$v \leftarrow$ last entry in $\edgestack$ \;
            remove last entry from $\edgestack$ \;
            $w \leftarrow$ a random vertex chosen with prob.\ proportional to $d^-_{\mathrm{unused}}(w)$\;
            $d^-_{\mathrm{unused}}(w)\leftarrow d^-_{\mathrm{unused}}(w)-1$ \tcp*[f]{we have paired an in-edge of $w$}\;
            add the edge $(v,w)$ to $M$\;
    }
    }
    
    \caption{The eDFS procedure \label{alg:edfs}}
\end{algorithm}

==> Content/Sections/lukasiewiczpathheightprocess.tex <==
Let $T=(V,E,\rho)$ be an ordered rooted finite tree with vertex set $V$, edge set $E$ and root $\rho$; say $|V|=n$. Let $v_0,\dots,v_{n-1}$ denote the vertices of the tree visited in depth-first order, so that $v_0$ is the root of the tree. We can view $T$ as a metric space by regarding all edges as line segments of length $1$ that are connected via the vertices. The distance $d_T$ between points $a_1$ and $a_2$ on line segments $l_1$ and $l_2$ respectively is then defined as the length of the unique non-self-intersecting path between $a_1$ and $a_2$ that traverses the line segments of the tree. Denote $(T,d_T)$ by $\mathrm{T}$.\\
We will define the height function and \L ukasiewicz path of $\mathrm{T}$. Both of these functions uniquely characterize $\mathrm{T}$. The height process of $\mathrm{T}$, referred to as $h$, is defined as $$h(i)=d_T(v_i,v_0),$$ i.e.  for all $i$, $h(i)$ equals the distance from $v_i$ to the root.
Moreover, for all $i=1,\dots,n$, let $y_i$ be the number of children of $v_{i-1}$, and set $y_0=1$. Then, the \L ukasiewicz path of $\mathrm{T}$ is defined by $$s(i)=\sum\limits_{j\leq i} (y_j-1)$$ for $i=0,\dots,n$. Then, $s(i)$ is the total number of younger siblings of $v_i$ and its ancestors.

Suppose we have a function $\ell:E\to [0,\infty)$. Then, we can view $T$ as a metric space by regarding an $e$ as a line segment with length $\ell(e)$. The metric $d_T^\ell$ is defined similarly to $d_T$, and we denote the resulting metric space $(T,d^\ell_T)$ by $\mathrm{T}^\ell$, and call it a \emph{ordered rooted finite tree with edge lengths}. This gives rise to an alternative height process, referred to as $h^\ell$, which is defined $$h^\ell(i)=d^\ell_T(v_i,v_0),$$ i.e.  for all $i$, $h^\ell(i)$ equals the distance from $v_i$ to the root in $\mathrm{T}^\ell$. We set the \L ukasiewicz path of $\mathrm{T}^\ell$ equal to the \L ukasiewicz path of $\mathrm{T}$.

For a sequence of ordered rooted finite trees (with or without edge lengths), we define its height process by concatenating the height processes of the trees in the sequence. The \L ukasiewicz path is defined similarly. 
